Cosmological Radiation Hydrodynamics with ENZO

We describe an extension of the cosmological hydrodynamics code ENZO to include the self-consistent transport of ionizing radiation modeled in the flux-limited diffusion approximation. A novel feature of our algorithm is a coupled implicit solution of radiation transport, ionization kinetics, and gas photoheating, making the timestepping for this portion of the calculation resolution independent. The implicit system is coupled to the explicit cosmological hydrodynamics through operator splitting and solved with scalable multigrid methods. We summarize the numerical method, present a verification test on cosmological Stromgren spheres, and then apply it to the problem of cosmological hydrogen reionization.

==> Makefile <==
#===========================================================================
# Make dependency file for LaTeX/BibTeX documents.
#===========================================================================
# To customize this makefile for use with another document, you will
# need to edit the macros in the first section, and to customize this
# makefile for use with other compilation programs, you will need to 
# edit the macros in the second section.
#
# Target   : the primary document name.
# TexFiles : lists actual names of files referenced in the primary document,
#            e.g. with LaTeX's \include command.
# FigFiles : lists names of figure files 
# BibFile  : lists actual names of .bib files referenced in your
#	     document with LaTeX's \bibliography command.
#
# Macros which exceed one line in length are joined with a backslash (\)
# at the end of the line. Macros with more than one value, e.g. multiple
# file names, must be surrounded by parentheses, either () or {}.
#===========================================================================

 Target   = paper
 TexFiles = introduction.tex physical_model.tex algorithm.tex \
            verification_tests.tex application_cosmo_ionization.tex \
	    conclusions.tex
 FigFiles = 
 BibFile  = sources.bib
 StyFiles = 
#===========================================================================
# LaTeX and BibTeX commands
#===========================================================================

 LaTeX      = latex
 BibTeX     = bibtex
 DVItoPS    = dvips
 DVItoPDF   = dvipdfm

#===========================================================================
# external program options
#===========================================================================

 Editor     = emacs
 PSview     = gv	
 PDFview    = acroread
 DVIview    = xdvi

#===========================================================================
# Archiving stuff
#===========================================================================

 Date       = $(shell date +%m.%d.%Y)
 ArkDir     = ${Target}-$(Date)
 ArkDirFull = ${Target}-all-$(Date)
 ArkFiles   = ${Target}.tex ${Target}.pdf $(TexFiles) $(BibFile) $(StyFiles) Makefile

#===========================================================================
# Targets, options, and dependencies
#===========================================================================

all:	${Target}.pdf

${Target}.pdf:	${Target}.dvi
	${DVItoPDF} ${Target}.dvi
	make clean

${Target}.ps:	${Target}.dvi
	${DVItoPS} ${Target}.dvi -o ${Target}.ps
	make clean

${Target}.dvi:	${TexFiles} ${FigFiles} ${StyFiles} ${Target}.tex ${Target}.bbl 
	${LaTeX} ${Target}
	${LaTeX} ${Target}

${Target}.bbl:	$(BibFile)
	${LaTeX} ${Target}
	${LaTeX} ${Target}
	${BibTeX} ${Target}


clean:
	rm -f "\#"*"\#" *.dvi *.aux *.log *.blg *.toc *.lof *.lot

realclean: clean
	rm -f *~ *.pdf *.ps

#===========================================================================
# Viewing and editing options
#===========================================================================

edit: ${Target}.tex
	${Editor} ${Target}.tex &

view: ${Target}.ps
	${PSview} ${Target}.ps &

read: ${Target}.pdf
	${PDFview} ${Target}.pdf &

xview: ${Target}.dvi
	${DVIview} ${Target}.dvi &

#===========================================================================
# Archive file options
#===========================================================================

# Create tar archive of latex sources (text files only)
archive: 
	make all
	make clean
	rm -Rf $(ArkDir)
	mkdir $(ArkDir)
	cp -R $(ArkFiles) $(ArkDir)
	tar -czf $(ArkDir).tgz $(ArkDir)
	rm -Rf $(ArkDir)

# Create tar archive of all sources
fullarchive: 
	make all
	make clean
	rm -Rf $(ArkDirFull)
	mkdir $(ArkDirFull)
	cp -R $(ArkFiles) $(FigFiles) $(ArkDirFull)
	tar -czf $(ArkDirFull).tgz $(ArkDirFull)
	rm -Rf $(ArkDirFull)


#===========================================================================
# End of Makefile
#===========================================================================

